Towards Training Billion Parameter Graph Neural Networks for Atomic Simulations

Recent progress in Graph Neural Networks (GNNs) for modeling atomic simulations has the potential to revolutionize catalyst discovery, which is a key step in making progress towards the energy breakthroughs needed to combat climate change. However, the GNNs that have proven most effective for this task are memory intensive as they model higher-order interactions in the graphs such as those between triplets or quadruplets of atoms, making it challenging to scale these models. In this paper, we introduce Graph Parallelism, a method to distribute input graphs across multiple GPUs, enabling us to train very large GNNs with hundreds of millions or billions of parameters. We empirically evaluate our method by scaling up the number of parameters of the recently proposed DimeNet++ and GemNet models by over an order of magnitude. On the large-scale Open Catalyst 2020 (OC20) dataset, these graph-parallelized models lead to relative improvements of 1) 15% on the force MAE metric for the S2EF task and 2) 21% on the AFbT metric for the IS2RS task, establishing new state-of-the-art results.

==> egn_block_dist.tex <==
\begin{enumerate}
    \item In each processor $p$ in parallel, update the representations for each triplet in $T^{(p)}$ in parallel using equation \ref{eq:triplet_update}.
    \item For each edge $k$, in each processor $p$, locally aggregate the triplet representations, followed by an all-reduce for global aggregation.
    \begin{equation} \label{eq:triplet_aggr}
    \begin{split}
        \Bar{\ttt}'^{(p)}_k &= \TA (T'^{(p)}_k) \\
        \Bar{\ttt}'_k &= \AllReduce ( \{ \Bar{\ttt}'^{(p)}_k \}_{p=1:P} )
    \end{split}
    \end{equation}
    At this stage, all processors have the aggregated representations $\Bar{\ttt}'_k$.
    
    \item In each processor $p$ in parallel, update the representations for each edge in $E^{(p)}$ in parallel using equation \ref{eq:edge_update}.
    \item For each node $i$, in each processor $p$, locally aggregate the edge representations, and then perform an all-reduce step to globally aggregate the edge representations.

    \begin{equation} \label{eq:edge_aggr}
    \begin{split}
        \Bar{\ee}'^{(p)}_i &= \EA (E'^{(p)}_i) \\
        \Bar{\ee}'_i &= \AllReduce ( \{ \Bar{\ee}'^{(p)}_i \}_{p=1:P} )
    \end{split}
    \end{equation}

    \item In each processor $p$ in parallel, update the representations for each node in $V^{(p)}$ using equation \ref{eq:node_update}.

    \item Finally, locally aggregate node representations, all-reduce the results and update the global attributes. 
    \begin{equation} \label{eq:node_update}
    \begin{split}
       \Bar{\vv}'^{(p)} &= \NA (V'^{(p)}) \\
       \uu' &= \GU (\Bar{\vv}', \uu)
    \end{split}
    \end{equation}
    where $V' = \{\vv'_i\}_{i=1:N^v}$.

\end{enumerate}


==> egn_block_seq.tex <==

\begin{enumerate}
    \item Update each triplet representation:
    \begin{equation} \label{eq:triplet_update}
        \ttt'_m = \TU (\ttt_m, \ee_{m_1}, \ee_{m_2}, \uu)
    \end{equation}
    \item For each edge $k$, aggregate the updated representations of all triplets involving edge $k$:
    \begin{equation} \label{eq:triplet_aggr}
        \Bar{\ttt}'_k = \TA (T'_k)
    \end{equation}
    where $T'_k = \{ (\ttt'_m, e_{m_1}, e_{m_2}) | e_{m_1} = k \}$.
    
    \item Update each edge representation using the aggregated triplet representations:
    \begin{equation} \label{eq:edge_update}
        \ee'_k = \EU (\ee_k, \vv_{r_k}, \vv_{s_k}, \Bar{\ttt}'_k, \uu)
    \end{equation}
    \item For each node $i$, aggregate the updated edge representations for all edges incident on node $i$:
    \begin{equation} \label{eq:edge_aggr}
        \Bar{\ee}'_i = \EA (E'_i)
    \end{equation}
    where $E'_i = \{ (\ee'_k, r_k, s_k) | r_k = i \}$.
    
    \item Update each node representation using the aggregated edge representations:
    \begin{equation} \label{eq:node_update}
        \vv'_i = \NU (\vv_i, \Bar{\ee}'_i, \uu)
    \end{equation}
    
    \item Finally, aggregate information from all the nodes and update the global attributes:
    \begin{equation} \label{eq:node_update}
      \Bar{\vv}' = \NA (V')
    \end{equation}
    \begin{equation} \label{eq:node_aggr}
      \uu' = \GU (\Bar{\vv}', \uu)
    \end{equation}
    where $V' = \{\vv'_i\}_{i=1:N^v}$
    
\end{enumerate}
